RAP: Robustness-Aware Perturbations for Defending against Backdoor Attacks on NLP Models

Backdoor attacks, which maliciously control a well-trained model's outputs of the instances with specific triggers, are recently shown to be serious threats to the safety of reusing deep neural networks (DNNs). In this work, we propose an efficient online defense mechanism based on robustness-aware perturbations. Specifically, by analyzing the backdoor training process, we point out that there exists a big gap of robustness between poisoned and clean samples. Motivated by this observation, we construct a word-based robustness-aware perturbation to distinguish poisoned samples from clean samples to defend against the backdoor attacks on natural language processing (NLP) models. Moreover, we give a theoretical analysis about the feasibility of our robustness-aware perturbation-based defense method. Experimental results on sentiment analysis and toxic detection tasks show that our method achieves better defending performance and much lower computational costs than existing online defense methods. Our code is available at https://github.com/lancopku/RAP.

==> tables/detection_results_apmf_frr1.tex <==
\begin{table}[t!]
\small
\centering
 \setlength{\tabcolsep}{4pt}
\sisetup{detect-all,mode=text}
\begin{tabular}{@{}lllrrr@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Target\\ Dataset\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Poisoned\\ Dataset\end{tabular}   &\begin{tabular}[c]{@{}l@{}}Attack\\ Method\end{tabular} & ASR &  FRR  & FAR \\
\midrule[\heavyrulewidth]
% imdb
\multirow{4.5}{*}{IMDB} & \multirow{2}{*}{Yelp} & RIPPLES&   98.44  & 1.04 & 0.62 \\
 & & BadNet-SL &  96.35 & 1.23 & 2.21   \\
 \cmidrule{2-6}
 & \multirow{2}{*}{Amazon} & RIPPLES &   98.60 & 1.04 & 8.86 \\
 & & BadNet-SL &  96.06  & 1.31 &0.57 \\
\cmidrule{1-6}
\multirow{2}{*}{Twitter} & \multirow{2}{*}{Jigsaw} & RIPPLES&   98.10 & 1.08 & 4.10 \\
 & & BadNet-SL &  100.00 & 1.35 & 0.00  \\
\bottomrule
\end{tabular}
\caption{Performance of RAP against RIPPLES and BadNet-SL in the setting where the backdoored model will be fine-tuned on a clean dataset before deployed. FRR on clean training samples is $1$\%.}
\label{tab: detection results APMF frr1}
\end{table}

==> tables/detection_results_apmf_full.tex <==
\begin{table*}[t!]
\centering
 \setlength{\tabcolsep}{5.5pt}
\sisetup{detect-all,mode=text}
\begin{tabular}{lllcrr}
\toprule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Target\\ Dataset\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Poisoned \\ Dataset\end{tabular}}   &\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Attack\\ Method\end{tabular}} &  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FRR (\%) \\on Training\\ Samples\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FRR (\%) \\on Testing \\Samples\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}FAR (\%) \\on Testing \\Samples\end{tabular}} \\
& & & & & \\
& & & & & \\
\midrule[\heavyrulewidth]
% imdb
\multirow{17}{*}{IMDB} & \multirow{8}{*}{Yelp} & \multirow{4}{*}{RIPPLES} &  0.5 & 0.5932 & 0.7680  \\
 &  &  &  1.0 & 1.0411 & 0.6160 \\
 &  &  &  3.0 & 3.0192 & 0.2800 \\
 &  &  &  5.0 &5.1796  & 0.1920 \\
 \cmidrule{3-6}
 &  & \multirow{4}{*}{BadNet-SL} &  0.5 & 0.6796 & 2.4656\\
 &  &  &  1.0 & 1.2305 & 2.2083 \\
 &  &  &  3.0 & 4.4339 & 1.7849 \\
 &  &  &  5.0 & 5.3745 & 1.6188 \\
 \cmidrule{2-6}
 & \multirow{8}{*}{Amazon} & \multirow{4}{*}{RIPPLES} &  0.5 & 0.4508 & 17.5760 \\
 &  &  &  1.0 & 1.0397 & 8.8640 \\
 &  &  &  3.0 & 3.0364 & 5.8640 \\
 &  &  &  5.0 & 4.9411 & 3.1680 \\
 \cmidrule{3-6}
 &  & \multirow{4}{*}{BadNet-SL} &  0.5 & 0.7876 & 0.6662 \\
 &  &  &  1.0 & 1.3113 & 0.5662 \\
 &  &  &  3.0 & 3.7813 & 0.5579 \\
 &  &  &  5.0 & 5.7997 & 0.5496 \\
 \midrule
 \multirow{8}{*}{Twitter} & \multirow{8}{*}{Jigsaw} & \multirow{4}{*}{RIPPLES} &  0.5 & 0.6499 & 9.4867 \\
 &  &  &  1.0 & 1.0833 & 4.1033 \\
 &  &  &  3.0 & 3.1121 & 1.8779 \\
 &  &  &  5.0 & 4.8257 & 0.9916 \\
 \cmidrule{3-6}
 &  & \multirow{4}{*}{BadNet-SL} &  0.5 & 0.7441 & 0.0000 \\
 &  &  &  1.0 & 1.3510 & 0.0000 \\
 &  &  &  3.0 & 3.1721 & 0.0000 \\
 &  &  &  5.0 & 5.1889 & 0.0000 \\
\bottomrule
\end{tabular}
\caption{Full results of RAP in the setting where the backdoored model will be fine-tuned on a clean dataset before deployed.}
\label{tab: detection results APMF full}
\end{table*}

==> tables/notations.tex <==
\begin{table}[t!]
\small
  \centering
  \sisetup{detect-all,mode=text}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}cc@{}}
    \toprule
    Notation & Definition \\
    \midrule
    $t^{*}$ & Backdoor trigger \\
    \midrule
    $\hat{t}$ & Our robustness-aware perturbation trigger \\
    \midrule
    $y_{T}$ & Target/protect label \\
    \midrule
    $\mathcal{D}$ & Clean data distribution \\
    \midrule
    $\mathcal{D}^{T}$ & \tabincell{c}{$\{ (x,y) \in \mathcal{D} | y=y_{T}\}$, \\clean samples whose labels are $y_{T}$} \\
    \midrule
    $f(x;\theta)$ & \tabincell{c}{Output of model $f$ with input $x$ and weights $\theta$} \\ 
    \midrule
    $\theta^{*}$ & Weights in a backdoored model \\
    \midrule
    $p_{\theta}(x;y)$ & \tabincell{c}{$\mathbb{P}(f(x;\theta) = y)$, the output probability\\ of class $y$ for input $x$ given by $f(\cdot; \theta)$} \\
    \bottomrule
  \end{tabular}
\caption{Notations and their definitions.}
\label{tab: notations}
 % \vskip -0.2 in
\end{table}
